Epistemic Modality and Coordination under Uncertainty

Communication facilitates coordination, but coordination might fail if there's too much uncertainty. I discuss a scenario in which vagueness-driven uncertainty undermines the possibility of publicly sharing a belief. I then show that asserting an epistemic modal sentence, 'Might p', can reveal the speaker's uncertainty, and that this may improve the chances of coordination despite the lack of a common epistemic ground. This provides a game-theoretic rationale for epistemic modality. The account draws on a standard relational semantics for epistemic modality, Stalnaker's theory of assertion as informative update, and a Bayesian framework for reasoning under uncertainty.

==> eptcsdata.tex <==
\providecommand{\firstpage}{295}
\providecommand{\publicationstatus}{J. Y. Halpern and A. Perea (Eds.): Theoretical Aspects \\
of Rationality and Knowledge 2021 (TARK 2021) \\
EPTCS 335, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.335.28}{10.4204/EPTCS.335.28}}

